Blackbox Attacks via Surrogate Ensemble Search

Blackbox adversarial attacks can be categorized into transfer- and query-based attacks. Transfer methods do not require any feedback from the victim model, but provide lower success rates compared to query-based methods. Query attacks often require a large number of queries for success. To achieve the best of both approaches, recent efforts have tried to combine them, but still require hundreds of queries to achieve high success rates (especially for targeted attacks). In this paper, we propose a novel method for Blackbox Attacks via Surrogate Ensemble Search (BASES) that can generate highly successful blackbox attacks using an extremely small number of queries. We first define a perturbation machine that generates a perturbed image by minimizing a weighted loss function over a fixed set of surrogate models. To generate an attack for a given victim model, we search over the weights in the loss function using queries generated by the perturbation machine. Since the dimension of the search space is small (same as the number of surrogate models), the search requires a small number of queries. We demonstrate that our proposed method achieves better success rate with at least 30x fewer queries compared to state-of-the-art methods on different image classifiers trained with ImageNet. In particular, our method requires as few as 3 queries per image (on average) to achieve more than a 90% success rate for targeted attacks and 1-2 queries per image for over a 99% success rate for untargeted attacks. Our method is also effective on Google Cloud Vision API and achieved a 91% untargeted attack success rate with 2.9 queries per image. We also show that the perturbations generated by our proposed method are highly transferable and can be adopted for hard-label blackbox attacks. We also show effectiveness of BASES for hiding attacks on object detectors.

==> notes.tex <==
The pros and cons of these methods are usually balancing between success rates and the number of queries. Some works have leveraged both for achieving higher success rates with less queries (cite some papers), including this paper. One way to improve the transferability of transfer-based attacks is to use an ensemble of different models as the surrogate . This method is intuitive, that if the adversarial image can fool multiple models, it is more likely to transfer to unseen models. (It is also practical in numerous cases, since different models keeps being developed for the same tasks, and the majority of new models are derived from existing models. There is a high chance that the model in deployment share some similarity with certain surrogate model in the ensemble. Cite the paper about fundamental models, which seems to advocate for this?. ) Current approaches for ensemble attacks usually use uniform weights for all the ensemble models, \i.e. each model has the same weight regardless of the victim model. However, we find that we can achieve higher success rate by optimizing the weights of ensemble models for different victim models, victim images, and target labels.

\paragraph*{Controlled perturbations for ensemble.} The space of perturbations that can fool a single model is often large. A single perturbation that can fool multiple surrogate models simultaneously lies at the intersection of all the individual perturbation spaces and expected to transfer to other models \cite{existing surrogate ensemble methods???}. Our main insight is that an arbitrary combination of surrogate models does not necessarily provide a perturbation that fools the victim model. Nevertheless, if the surrogate ensemble is diverse enough and our PM can generate perturbations in a conrollable manner, then we can steer the perturbations to fool the victim model. This effect is illustrated in Figure~\ref{fig:intro}. 


\Salnote{This para can probably go to related work}
Reducing the dimension of the search space for query-based attacks is an active area of research \cite{???} because gradient estimation over a $\mathcal{D}$-dimensional parameter requires $O(\mathcal{D})$ queries. We summarize the typical search space and average number of queries for some of the existing methods in Table~\ref{tab:pros-cons}.
Direct search over the image space requires as many queries as the number of pixels (e.g., $224\times224\times3 = 150,528$ for a typical image in ImageNet dataset) in the worst case, which is infeasible.  
P-RGF \cite{} leverages data-dependent priors and draw random vectors from a subspace of $50\times50\times3 = 7,500$. SimBA-DCT \cite{} searches over the first \nicefrac{1}{8} of DCT frequencies, reducing the dimension to $28\times28\times3 = 2,352$. TREMBA \cite{} trains a perturbation generator and searches over the latent space with a dimension of $8\times14\times14 = 1,568$. GFCS uses ODS approach \cite{} which randomly samples over logit space of dimension $1000$. In our approach, we further shrink the search dimension to as low as the number of models in the ensemble. In our experiments, we show that a moderate-size ensemble with $20$ models can generate successful attacks for a variety of victim models while requiring (on average) 3 queries than existing methods. \Salnote{We probably need some specific numbers} 
